Robust and leakage-resilient device-independent oblivious transfer in MiniQCrypt

Assuming post-quantum one-way functions, we construct device-independent oblivious transfer and bit commitment that tolerate independent honest faults at a constant rate and adaptive, bidirectional quantum leakage between the laboratories at a constant rate. Honest parties use trusted classical computation to operate untrusted quantum devices, which may share arbitrary entanglement and perform joint measurements without assumptions of independence or identical distribution. Security is simulation-based against quantum polynomial-time adversaries and composes sequentially with efficient simulators. For security parameter $\lambda$ and a prescribed total leakage budget $\ell$, one complete one-bit oblivious transfer uses $\Theta(\ell+\log^2\lambda)$ device coordinates in at most three single-use device windows, including preprocessing, and polynomial classical computation and communication. The leakage budget is shared across these windows. The commitment has efficient simulators against both parties and yields device-independent coin tossing with abort; each uses one window. Completeness of oblivious transfer gives device-independent secure computation with abort for every efficiently computable classical functionality on a fixed number of parties, against static corruption of any proper subset, provided each reached call to oblivious transfer satisfies the device and budget conditions. The construction combines short selectors with code-based choice masking, a global audit, and error correction across field symbols. The commitment extractor changes a classical code coset while leaving the device execution and its leakage unchanged. Sender security uses a global Fourier analysis and a selector-aware Magic Square repetition bound derived from the two-round threshold theorem of Kundu and Tan (2023).

==> preamble.tex <==
% REVISION-ID: PREAMBLE 2026-10-13-predicate-fonts
% Shared preamble: packages, theorem environments, and notation.
\newif\ifdiotlncs
\makeatletter
\@ifclassloaded{llncs}{\diotlncstrue}{\diotlncsfalse}
\makeatother

% Encoding and page layout
\usepackage[utf8]{inputenc}
\usepackage[T1]{fontenc}
\ifdiotlncs\else
\usepackage[letterpaper,margin=1in]{geometry}
\fi

% Mathematics and fonts
\usepackage{amssymb}
\usepackage{amsfonts}
% llncs defines \vec incompatibly with the amsmath stack loaded by mathtools.
\ifdiotlncs
\makeatletter
\expandafter\let\csname vec \endcsname\@undefined
\let\vec\@undefined
\DeclareMathAccent{\vec}{\mathord}{letters}{"7E}
\makeatother
\fi
\usepackage{mathtools}
\ifdiotlncs\else
\usepackage{amsthm}
% Computer Modern, in its scalable Latin Modern form (T1 encoding needs it).
\usepackage{lmodern}
\fi
\usepackage{braket}
\usepackage{scalerel}

% Tables and formatting
\usepackage{xcolor}
\usepackage{graphicx}
\usepackage{float}
\usepackage[shortlabels]{enumitem}
\usepackage{array}
\usepackage{arydshln}

% References: cleveref must be loaded after hyperref.
\usepackage{thmtools}
\usepackage{hyperref}
\hypersetup{colorlinks=true,
  linkcolor={blue!50!black},   % cross-references: theorems, sections, protocols, equations
  citecolor={green!35!black},  % citations
  urlcolor={blue!50!black}}
\usepackage[nameinlink,capitalize,noabbrev]{cleveref}
\usepackage{placeins}
\usepackage[protrusion=false]{microtype}
\usepackage{tikz}
\usetikzlibrary{arrows.meta,positioning,calc}

% Theorem environments.  LNCS supplies theorem, lemma, definition, and proof.
\ifdiotlncs
\spnewtheorem{cor}[theorem]{Corollary}{\bfseries}{\itshape}
\spnewtheorem{fact}{Fact}{\bfseries}{\itshape}
\let\claim\relax
\let\endclaim\relax
\spnewtheorem{claim}{Claim}{\bfseries}{\itshape}
\else
\newtheorem{theorem}{Theorem}
\newtheorem{lemma}{Lemma}
\newtheorem{cor}[theorem]{Corollary}
\newtheorem{fact}{Fact}
\newtheorem{claim}{Claim}

\theoremstyle{definition}
\newtheorem{definition}{Definition}
\theoremstyle{plain}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem*{theorem*}{Theorem}
\theoremstyle{remark}
\newtheorem{remark}[theorem]{Remark}
\fi

\crefname{fact}{Fact}{Facts}
\Crefname{fact}{Fact}{Facts}
\crefname{claim}{Claim}{Claims}
\Crefname{claim}{Claim}{Claims}

% Number a single line inside an unnumbered display.
\newcommand{\numberthis}{\addtocounter{equation}{1}\tag{\theequation}}

% Basic mathematical notation
\newcommand{\poly}{\mathrm{poly}}
\newcommand{\abs}[1]{\left|#1\right|}
\newcommand{\floor}[1]{\left\lfloor#1\right\rfloor}
\newcommand{\eps}{\varepsilon}
\newcommand{\Id}{\mathbb{I}}
\newcommand{\emptystring}{{\scaleto{\emptyset}{8pt}}}
\newcommand{\wht}[1]{\widehat{#1}}

\DeclareMathOperator{\Tr}{Tr}
\newcommand{\D}{\operatorname{D}}
\newcommand{\I}{\operatorname{I}}
\renewcommand{\S}{\operatorname{S}}

% States, inner products, and distances
\newcommand{\ketbra}[2]{\ket{#1}\!\bra{#2}}
\newcommand{\kb}[1]{\ketbra{#1}{#1}}
\newcommand{\junkstate}{\ket{\mathtt{junk}}}
\newcommand{\norm}[1]{\ensuremath{\left\lVert #1\right\rVert}}
\newcommand{\onenorm}[2]{\left\lVert #1-#2\right\rVert_1}
\newcommand{\paren}[1]{\left(#1\right)}
\newcommand{\brak}[1]{\left\{#1\right\}}
\newcommand{\diver}[2]{\D\!\left(#1\middle\|#2\right)}

\newcommand{\defeq}{\coloneqq}
\newcommand{\mcL}{\mathcal{L}}
\DeclareMathOperator*{\Exp}{\mathbb{E}}
\newcommand{\wt}{\operatorname{wt}}
\newcommand{\subdist}{\operatorname{Sub}}

% Cryptographic notation
\newcommand{\adv}{\mathsf{Adv}}
\newcommand{\negl}{\operatorname{negl}}
\newcommand{\polylog}{\operatorname{polylog}}
\newcommand{\alice}{\mathsf{Alice}}
\newcommand{\bob}{\mathsf{Bob}}
\newcommand{\sfA}{\mathsf{A}}
\newcommand{\sfB}{\mathsf{B}}
\newcommand{\device}{\mathbf{D}}
\newcommand{\MS}{\textup{MS}}

\newcommand{\Sim}{\textnormal{\textsc{Sim}}}
\newcommand{\ideal}{\textnormal{\textsc{ideal}}}
\newcommand{\Com}{\textnormal{\textsc{Commit}}}
\newcommand{\Rev}{\textnormal{\textsc{Reveal}}}
\newcommand{\sdec}{\textnormal{\textsc{SyndDec}}}
\newcommand{\ext}{\mathsf{Ext}}

\renewcommand{\H}{\operatorname{H}}
\newcommand{\hmin}{\mathrm{H}_{\min}}

% Protocol-table spacing
\newcommand{\tab}{\hspace{2cm}}

% Comments
\newcommand{\RJnote}[1]{\textcolor{red}{\small {\textbf{(Rahul:} #1\textbf{) }}}}
% Scope the color locally while allowing paragraph breaks in the note.
\newcommand{\Ynote}[1]{{\color{red}\small\textbf{(YaoNan:} #1\textbf{) }}}
\newcommand{\ZCnote}[1]{\textcolor{blue}{\small {\textbf{(Zhili:} #1\textbf{) }}}}

% Paper-specific environments, floats, and notation (used by the paper and the extended abstract).
\ifdiotlncs\else
% Keep the abstract at the submission's normal 11-point size.
\renewenvironment{abstract}{%
  \begin{center}\bfseries\abstractname\end{center}%
  \noindent\ignorespaces}{\par}
\fi

% Protocols and simulators use one boxed algorithmica float throughout.
\floatstyle{boxed}
\newfloat{algorithmica}{htbp}{loa}
% A boxed procedure that may break across pages. It takes the caption
% and the counter of the algorithmica float, so numbering is continuous.
\usepackage{caption}
\usepackage[most]{tcolorbox}
\newenvironment{protocolbox}{%
  \begin{tcolorbox}[breakable,enhanced,sharp corners,colback=white,
    colframe=black,boxrule=0.4pt,left=4pt,right=4pt,top=4pt,bottom=4pt,
    before skip=8pt plus 2pt,after skip=4pt]}{\end{tcolorbox}}
\floatname{algorithmica}{Protocol}
\floatstyle{plain}
\crefname{algorithmica}{protocol}{protocols}
\Crefname{algorithmica}{Protocol}{Protocols}
% Continuations share the preceding protocol number and have distinct PDF targets.
\newcommand{\continuedprotocol}[1]{%
  \addtocounter{algorithmica}{-1}%
  \renewcommand{\thealgorithmica}{\arabic{algorithmica}, Part~#1}%
  \def\theHalgorithmica{\arabic{algorithmica}.part.#1}}
\newcommand{\OTprotocolparts}{\Cref{prot:di-ot}}

% A common float, type size, spacing, and numbered-step style for procedures.
\newcommand{\protocolstyle}{\normalsize
  \setlength{\tabcolsep}{3pt}\renewcommand{\arraystretch}{1.08}}
\newenvironment{protocolsteps}{\begin{enumerate}[
  label=\textnormal{\arabic*.},leftmargin=1.8em,itemsep=3pt,
  topsep=3pt,parsep=0pt]}{\end{enumerate}}
\newcommand{\Syn}{\mathsf{Syn}}
\newcommand{\Dec}{\mathsf{Dec}}

\newcommand{\EqCom}{\mathsf{EqCom}}
\newcommand{\EqCommit}{\mathsf{EqCommit}}
\newcommand{\EqOpen}{\mathsf{EqOpen}}
\newcommand{\Ver}{\mathsf{OpenVer}}
\newcommand{\Mode}{\mathsf{MODE}}
\newcommand{\Label}{\mathsf{LABEL}}
\newcommand{\Pay}{\mathsf{PAY}}
\newcommand{\Acc}{\mathsf{Acc}}
\newcommand{\QPT}{\mathsf{QPT}}
\newcommand{\ind}{\mathbf 1}
\newcommand{\Ftwo}{\mathbb F_2}
\newcommand{\Zthree}{\mathbb Z_3}
\newcommand{\Rref}{\mathcal R}
\newcommand{\Eqa}{\mathsf E_{\!A}}
\newcommand{\Eqb}{\mathsf E_{\!B}}
\newcommand{\kpad}{k_{\mathrm{pad}}}
\newcommand{\ksel}{k_{\mathrm{sel}}}
\newcommand{\pg}{p_{\mathrm{guess}}}
\newcommand{\Bin}{\operatorname{Bin}}
\newcommand{\naud}{n_{\mathrm{aud}}}
\newcommand{\OpenAcc}{\mathsf{OpenAcc}}
\newcommand{\hY}{\widehat Y}
\newcommand{\tR}{\widetilde R}
\newcommand{\taudec}{\tau_{\mathrm{dec}}}
\newcommand{\tauopen}{\tau_{\mathrm{open}}}
\newcommand{\betasel}{\beta_{\mathrm{sel}}}
\newcommand{\csel}{c_{\mathrm{sel}}}
\newcommand{\Xraw}{X^{\mathrm{in}}}
\newcommand{\Araw}{A^{\mathrm{in}}}

% Multiplicative codes and their secret maps.
\newcommand{\Ffield}{\mathbb F_{64}}
\newcommand{\CodeA}{\mathcal A}
\newcommand{\CodeB}{\mathcal B}
\newcommand{\CodeD}{\mathcal D}
\newcommand{\secmap}{\operatorname{sec}}

